Semi-Offline Reinforcement Learning for Optimized Text Generation

In reinforcement learning (RL), there are two major settings for interacting with the environment: online and offline. Online methods explore the environment at significant time cost, and offline methods efficiently obtain reward signals by sacrificing exploration capability. We propose semi-offline RL, a novel paradigm that smoothly transits from offline to online settings, balances exploration capability and training cost, and provides a theoretical foundation for comparing different RL settings. Based on the semi-offline formulation, we present the RL setting that is optimal in terms of optimization cost, asymptotic error, and overfitting error bound. Extensive experiments show that our semi-offline approach is efficient and yields comparable or often better performance compared with state-of-the-art methods.

==> src/method_bak.tex <==
\section{Masked Semi-Offline}

【说明为什么要设计新方法，并从MLM引出semi-offline，因为MLM大家比较容易理解和接受】
Online需要费时的decoding, 这在大模型中尤其严重。Offline的方法可以避免costly online decoding processes，但也放弃了exploration的能力。我们不妨考虑是否存在设置可以同时避免costly online decoding也能具有exploration能力的方法。
受启发于MLM，我们是否可以类似MLM固定一个句子的一部分，并且探索其余部分？在MLM的设置下，我们可以保持模型的探索能力，同时将forward passing的次数降到最少。

【是不是证明结束再写这个MDP】
我们可以为MLM定义如下MDP:
\textit{STATE}: the state $s_t$ represents the input sequence x and the generated tokens, together with the masked position.
the generated tokens come from the dataset or the model.
$s_t=(x_1,\cdots,x_|x|,\hat{y_1}, y_2, \cdots, \hat{y}_t, m_1, m_2, \cdots, m_t)$

\textit{Action}: The MDP has a two-step action. Given state $s_t$, the policy will decide if the current position is masked. If masked, then it will be a predicted token, otherwise, it is a token from data.

\textit{Transition}: $s_{t+1}$=$\mathcal{T}(s_t, a_t)$\\=$(x_1,\cdots,x_|x|,y_1, y_2, \cdots, y_t, y_{t+1}, m_1, m_2, \cdots, m_t, m_{t+1})$

\textit{Reward}: The reward function R($s_t, a_t$) takes the sequence of tokens as input and it can be any sentence-evaluation tool, such as ROUGE and BLEU.

我们可以把MLM formulate成以下policy:
\begin{eqnarray}
(1-\alpha)p(y^D_i)+(1-\alpha) p(y|x^D,\hat{y}) \\
\hat{y}={y^D_j[M_j=0]+[MASK][M_j=1]},j<i 
\end{eqnarray} % to update MLM + policy

从串行的角度，在每个时间步，agent依照policy选择在当前序列填入data或者是填入自身的预测。同时，从MLM的角度，其可以实现时间友好的并行生成，但是并行生成也会带来一些牺牲，比如时序信息。
尽管MLM是一个被广泛使用的方法，但我们需要考虑其是否足够适合我们的场景。
我们接下来根据我们的desired properties给出可行方法定义，并证明MLM是一个满足给出定义的最简单的方法，并借助定义说明并行生成存在的问题和解决途径。
% （1）满足DP1和DP2
% 【怎么定义DP1，DP2，offline符合2不符合1，online符合1不符合2，semi-offline符合1和2。强调我们之前就强调的exploration和time cost两个点】
% We first give the definition of the desired methods.
% \begin{definition}[Basic]
% The generation procedure can be regard as a MDP.
% \label{dp0}
% \end{definition}

% % DP0 （basic）the generation procedure can be regard as a MDP。
% % 需要统一成token还是action to discuss
% \begin{definition}[Exploration] 
% The action of the agent can be a sampled token according to its own prediction. At time step t, the action is $a_t$ $\sim$ $p(y_t|X,Y<t,\theta)$
% \label{dp1}
% \end{definition}



% \begin{definition}[time cost] 
% % Assuming there is more than one token to be predicted by the agent, the prediction of the agent can be determined concurrently.
% % $a_i$ $\sim$ $p(y_i|X,Y<i,\theta)$ and
% % $a_j$ $\sim$ $p(y_j|X,Y<j,\theta)$ can be sampled concurrently.
% % Assuming there is more than one token for $Y$, any pair of the actions can be determined concurrently.
% The input of agent is determined concurrently and the actions of the agent is determined concurrently.
% \label{dp2}
% \end{definition}
% [输入要分两步，那就不是O(1),输出要分两步，也不是O(1)]


% % \begin{theorem}
% % When a method satisfies Definition ~\ref{dp0}, Definition ~\ref{dp1}, and Definition ~\ref{dp2}, the input of agent ≠ state. 
% % \end{theorem}

% \begin{theorem}
% When a method satisfies Definition ~\ref{dp0}, Definition ~\ref{dp1}, and Definition ~\ref{dp2}, the input of agent ≠ state. 
% \end{theorem}

% 定理1：依分布下，模型的输入H不包含做exploration的token. $H \neq S$, 对于分布函数F，也就是
% \begin{eqnarray}
% F_H(x) \neq F_S(x), \forall x    
% \end{eqnarray}

% 即模型输入中部分token与环境中真实存在的state中的token不同，模型只能看到部分真实的state.

% 证明：
% 根据定义3中，对任意$i$,$j$, 且$a_i=y_i,a_j=y_j$可以同时被决定, 不妨令$i<j$ 那么$a_i$,$a_j$的决定顺序是任意的，假设$a_j$先于$a_i$决定，根据定义2，$a_i$的结果具有随机性，而预测$a_j$的模型input具有确定性，那么$a_j$必定不能在输入上准确观测到$a_i$. 根据定义1，在时刻$j$，$s_j=(X,y_1, \cdots, y_i,\cdots,y_{j-1})$. $p(y_j|X,Y_{<j},\theta)$表示模型的输出的$y_j$的概率分布，其中X和$Y_{<j}$表示模型的输入，且$y_j \sim p(y|X,Y_{<j},\theta)$. 在$j$时刻，对输入而言，存在 $i$时刻无法被准确观测，那么$p(y|x,y,\theta)$中模型的输入(X,Y)不可能恒等于$s_j$中的(X,Y). 
% % [比如换词]
% % We define $H_{t}$ as the agent input for time step t. 
% 证明2:
% 对于任意$i<t$,$ \{y_i\}$ 是定义2中，按模型预测随机采样的token的集合，即做exploration的tokens.
% 假设$H_{t}$依照分布存在exploration token. 即$\{y_i\}$中存在任意exploration token $y_k$. 那么令$\hat{y_k}$是$s_t$中第k个token, $y_k$为 $H_{t}$第k个token，那么$\hat{y_k}$=$y_k$依分布相等，$\hat{y_k} \sim p(y_k|X,Y<k,\theta)$, 由于定义3，模型输入是确定的，$p(y_k)=1$, 该等式只在$p(\hat{y}_k|X,Y<k,\theta)=1$情况下成立，与定义2违背，在该情况下，$y_k$是确定的. 无法根据其分布进行exploration.



% % 【比如原本下一个输入了一个token，上一个位置的输出刚好sample到这个token，采样结果可能相等. 】
% 【这个证明也说明了exploration位置只有一个的情况，
% 跟昨天写那个的区别是，昨天是说生成token是随机的，输入是确定，所以S!=输入,这里是说如果随机token的分布和确定token分布相等会怎么样】
% 【需要在exploration定义里面加一条p!=1的限制
% 不然p(y)恒等于1的话，也不叫exploration?】

% 根据定义3中，对任意$i$,$j$, 且$a_i=y_i,a_j=y_j$可以同时被决定, 不妨令$i<j$ 那么$a_i$,$a_j$的决定顺序是任意的，假设$a_j$先于$a_i$决定，根据定义2，$a_i$的结果具有随机性，而预测$a_j$的模型input具有确定性，那么$a_j$必定不能在输入上准确观测到$a_i$. 根据定义1，在时刻$j$，$s_j=(X,y_1, \cdots, y_i,\cdots,y_{j-1})$. $p(y_j|X,Y_{<j},\theta)$表示模型的输出的$y_j$的概率分布，其中X和$Y_{<j}$表示模型的输入，且$y_j \sim p(y|X,Y_{<j},\theta)$. 在$j$时刻，对输入而言，存在 $i$时刻无法被准确观测，那么$p(y|x,y,\theta)$中模型的输入(X,Y)不可能恒等于$s_j$中的(X,Y). 

% 【有一点是其实$y_j$对前面的每个位置的预测的概率分布可能都清楚，所以唯一缺少的信息就是随机采样的结果未知】
% \begin{proof}

% % $state = {x1, \cdots, x_|x|, y_1, \hat{y}_2, \hat{y}_3, \cdots}$
% % If the input of the agent = state. then $\hat{y}_3$ $\sim$ $p(y|x, y_1, \hat{y}_2, \theta)$
% % [这样不严谨是因为这样也可以满足y2y3独立，需要加个前提，y3的前缀y变化会改变$p(y|x,y,\theta)$]

% % assuming there is a $y_i$, after 
% % the input of the agent


% % We define the input of the model as $o=(w^o_1,w^o_2, \cdots, w^o_T)$. s is the state of MDP.
% % % If Observation(t+1) = state(t+1)
% % No matter if o and s are the same， the agent can compute several token distributions $p(o_1), p(o_2),\cdots, p(o_T)$, and draw a token from the distribution(Definition ~\ref{dp1})， the sampled results of which are $W^o_1, W^o_2, \cdots, W^o_T$
% % % According to Definition ~\ref{dp2} \Rightarrow $p(o_i)$ can be computed regardless of the computing order \Rightarrow 
% % According to Definition ~\ref{dp2}, $p(o_i)$ can be computed regardless of the computing order, then we have:
% % \begin{eqnarray}
% % p(o_i) \perp\!\!\!\!\perp p(o_j),i\neq j \\ 
% % W^o_i \perp\!\!\!\!\perp W^o_j,i\neq j
% % \label{eq:depend}
% % \end{eqnarray}

% % According to Definition ~\ref{dp0}, we have  
% % \begin{equation}
% % s_{t+1} = \mathcal{T}(s_{t}, a_{t}), a_{t} \sim p(s_t)
% % \end{equation}
% % Where $a_t$ is the token drawn from the token distribution $p(s_t)$. $\mathcal{T}(s_{t}, a_{t})$ is the transition function, e.g., appending the token $a_t$ to the current sequence $s_t$.

% % Assuming $s_t$ = $o_t$, then we have $o_{t+1} = \mathcal{T}(o_{t}, a_{t}), a_{t} \sim p(o_t)$ and
% % $p(o_{t+1})=p(\mathcal{T}(o_{t}, a_{t})), a_{t} \sim p(o_t)$
% % This equation means there is a mapping from $w^o_t(a_t)$ to $p(o_{t+1})$,  the distribution of $w^o_{t+1}$. It will disobey Eq.~\ref{eq:depend}, as  $w^o_{t+1}$ dependent on $w^o_t$ and with the assumption of $s_t$ = $o_t$.
% \end{proof}



% DP3(逻辑说明在Theorem 1的问题下，如何解决这个问题，1.替换位置信息要被模型看到2.要借助belief state)
% 根据DP2，因为随机性和确定性的差别，模型输入在这种设置下一定无法准确地等于state，如果模型输入考虑随机性，$f_{\phi}$将raw input作为输入估计输出的期望作为模型$G_{\theta}$输入，那么模型输入可以与state近似的相等。
% 即在t时刻，

% \begin{eqnarray}
% E(X^{input},Y^{input}_{<t}))=E(X^S,Y^S_{<t})).    
% \end{eqnarray}

% \begin{eqnarray}
% E(X^{input},f_{\phi}(Y^{raw}_{<t}))=E(X^S,Y^S_{<t})).    
% \end{eqnarray}

% \begin{eqnarray}
% ||E(X^{input},Y^{input}_{<t}))-E(X^S,Y^S_{<t}))|| \leq \epsilon \\
% ||E(Y^{input}_{<t}))-E(Y^S_{<t}))|| \leq \epsilon  \\ 
% ||E(f_{\phi}(Y^{raw}_{<t})))-E(Y^S_{<t}))|| \leq \epsilon  \\ 
% \end{eqnarray}


% 接下来证明为了满足上式，一定需要满足条件1.位置信息已知，即对替换位置采样结果已知 2.对于T时刻，t<T的位置t的预测分布$p(y|X,Y_{<t},\theta)$可以近似估计。

% 考虑位置和概率分布具有随机性，对于任意$i,j(i<j)$,
% $y_i$服从的分布是
% $\beta \times p({y_{data}})+ (1-\beta)p(y|X,Y_{<i},\theta)$
% 其中$\beta$是二项分布p($\beta$)的参数。

% 1.由于$p(y|X,Y_{<i},\theta)$的输入和参数被$p(y|X,Y_{<j},\theta)$包含，我们可以先认为$p(y|X,Y_{<i},\theta)$对$p(y|X,Y_{<j},\theta)$而言是能够准确估计的。
% 2.假设$y_j$无法观测到$y_i$进行二项分布采样的结果，那么$y_j$需要估计$p(y^{data}_j)$,与$p(y|X,Y_{<i},\theta)$容易预测不同, agent对 $p(y^{data}_j|X,Y_{<i},\theta)$的估计是难以准确的，因为其原本分布是$p(y^{data}_j|Y^{data}_{<j})$.
% 且在训练过程中$p(y^{data})$实际上是一个确定的采样。
% 如果无法观测二项分布结果，那么上式期望等式很难成立。

% 我们的MLM，给出了符合DP3的最简信息，即二项分布采样结果，并且transformer的多层attention结构也使得
% $p(y|x,y<i,\theta)$的信息可以被$p(y|x,y<j,\theta)$利用。


